How Do Developers Use Code Suggestions in Pull Request Reviews?

GitHub introduced the suggestion feature to enable reviewers to explicitly suggest code modifications in pull requests. These suggestions make the reviewers' feedback more actionable for the submitters and represent a valuable knowledge for newcomers. Still, little is known about how code review suggestions are used by developers, what impact they have on pull requests, and how they are influenced by social coding dynamics. To bridge this knowledge gap, we conducted an empirical study on pull requests from 46 engineered GitHub projects, in which developers used code review suggestions. We applied an open coding approach to uncover the types of suggestions and their usage frequency. We also mined pull request characteristics and assessed the impact of using suggestions on merge rate, resolution time, and code complexity. Furthermore, we conducted a survey with contributors of the studied projects to gain insights about the influence of social factors on the usage and acceptance of code review suggestions. We were able to uncover four suggestion types: code style suggestions, improvements, fixes, and documentation with improvements being the most frequent. We found that the use of suggestions positively affects the merge rate of pull requests but significantly increases resolution time without leading to a decrease in code complexity. Our survey results show that suggestions are more likely to be used by reviewers when the submitter is a newcomer. The results also show that developers mostly search suggestions when tracking rationale or looking for code examples. Our work provides insights on the usage of code suggestions and their potential as a knowledge sharing tool.

==> tables/actions_per_edit_script.tex <==
\begin{table}
  \caption{Number of Actions per Edit Script}
  \label{tab:actions_edit_script}
  \begin{tabular}{lcc}
    \toprule
\textbf{\#Actions} & \textbf{Count} & \textbf{\%}\\
\midrule
0&425&9.92\%\\
1&1892&44.17\%\\
2&940&21.95\%\\
3&286&6.68\%\\
4&169&3.95\%\\
5&105&2.45\%\\
6&71&1.66\%\\
7&56&1.31\%\\
8&61&1.42\%\\
9&71&1.66\%\\
>=10&24&4.77\%\\
\midrule
Total&4755&100\\
  \bottomrule
\end{tabular}
\end{table}

==> tables/code_change_patterns.tex <==
\begin{table*}
  \caption{Code change patterns extracted from the  suggestions.}
  \label{tab:code_patterns}
  \begin{tabular}{llrrrrrl}
    \toprule
&\textbf{AST pattern (Action, Node) }&\textbf{C++}&\textbf{C\#}&\textbf{C}&\textbf{Python}&\textbf{Java}&\textbf{Description}\\
&&n=997&n=1835&n=74&n=544&n=833&\\
\toprule
1&-&10.4\%\cellcolor{red!25}&10.4\%&6.8\%&11\%&7.8\%&modify formatting\\
2&\{(I, specifier)\}&5.4\%&1.7\%&0\%&0\%&0\%&add specifier\\
3&\{(U, comment)\} or \{(U, TextElement)\}&5.9\%&\cellcolor{red!25}16.7\%&\cellcolor{red!25}29.7\%&0\%&\cellcolor{red!25}16.1\%&modify comment\\
4&\{(D, param), (I, parameter)\} or \{(D, argument), (I, argument)\}&3.6\%&2.7\%&0\%&1.3\%&0\%&replace argument\\
5&\{(D, decl\_statement), (I, decl\_statement)\}&2.4\%&0\%&0\%&0\%&0\%&replace variable declaration\\
6&\{(U, literal)\} or \{(U, StringLiteral)\} or \{(U, string)\}&6.5\%&3.3\%&4.1\%&12\%&11.9\%&modify literal\\
7&\{(U, name)\} or \{(U, SimpleName)\}&7.5\%&12.2\%&6.8\%&6.8\%&11.9\%&rename function/variable\\

8&\{(I, SimpleType)\}&0\%&0\%&0\%&0\%&1.6\%&specify class inheritance\\
9&\{(D, simple\_stmt), (I, simple\_stmt)\} or &3.3\%&0\%&0\%&\cellcolor{red!25}12.7\%&3.2\%&replace statement\\
&\{(D, expr\_stmt), (I, expr\_stmt)\} or&&&&&\\
&\{(D, ExpressionStatement), (I, ExpressionStatement)\}&&&&&&\\
\midrule
&\textbf{Total}&45.1\%&47\%&47.3\%&43.8\%&52.5\%&\\
\bottomrule
\end{tabular}
\end{table*}

==> tables/cognitive_complexity_total.tex <==
\begin{table*}[]
    \centering
    \begin{tabular}{r|r|r|r|r|r}
    \toprule
         \textbf{increase count (\%)} & \textbf{mean increase} & \textbf{decrease count (\%)} & \textbf{mean decrease} & \textbf{unchanged count (\%)} & \textbf{total count}\\
         \midrule
44 (1.93\%)& 3.48 & 123 (5.41\%)& -1.86 & 2107 (92.66\%)& 2274\\
\bottomrule
    \end{tabular}
    \caption{Cognitive Complexity Overall Changes}
    \label{tab:my_label}
\end{table*}

==> tables/lda_tpic_themes.tex <==
\begin{table*}
  \caption{Distribution of topic by emerging themes}
  \label{tab:freq}
  \begin{tabular}{lcll}
    \toprule
\textbf{Theme} & \textbf{\# Topics} & \textbf{Description}&\textbf{Selected keywords}\\
\midrule
Code Style & 6 &\makecell[l]{Alternative solution reflecting common or project-specific\\ code style conventions or reviewer preference} & \makecell[l]{convention, whitespace, style\_nitpick,comment, pattern,\\ consistent, rest, comma, trail, require}\\
\hline

Simplification & 5 & \makecell[l]{An alternative solution that simplifies\\ the code without changing its functionality\\ or eliminates unnecessary code}& \makecell[l]{instead, consider, unnecessary, simple, native,\\ slightly, retouch, concise, preferable, solution}\\
\hline

Avoiding Confusion & 3 &\makecell[l]{Points out possible confusions \\ or misunderstandings that might be\\ introduced by the code \\and proposes a less ambiguous version} & \makecell[l]{look\_like, sound, actually, original, mean,\\ confusing, simplify, believe, explicitely, implicit}\\
\hline
Fix & 2 &\makecell[l]{Points to potential side-effects or compilation\\problems arising from the code and proposes a fix}& \makecell[l]{avoid, property, problem, perform, instance,\\ compiler, prevent, generate, separate, paste}\\
\hline
Readability & 2 &\makecell[l]{Points to effort put into reading or comprehending\\ the code or future effort for other developers\\ and proposes a solution to reduce that effort }& \makecell[l]{read, easy, code, clear, think,\\understand, describe, explicit, suggest, scope}\\
\hline
Testing & 1 &\makecell[l]{Discusses ways to test the code portion\\ or warns about potential testing problems\\ and proposes a solution to foster testability}& \makecell[l]{test, break, change, block, object,\\ assume, performance, machine, subtle, able}\\
  \bottomrule
\end{tabular}
\end{table*}

==> tables/repositories_description.tex <==
\begin{table*}[b]
    \centering
% \vspace{0.2cm}
    \caption{Repositories under Study}
% \vspace{0.2cm}
    \begin{tabular}{llrr rrr rr}
    \toprule
         \textbf{Nr} & \textbf{Project} & \textbf{Forks} & \textbf{Size} & \textbf{Years} & \textbf{Primary Lang.} & \textbf{PRs (w/ Sugg.)*} & \textbf{Suggestions}\\
         \midrule
1 & dotnet/roslyn & 3108 & 1048.75 MB & 6 & C\# (66\%)  &9854  (660) & 1945 \\
2 & apache/flink & 7707 & 303.04 MB & 7 & Java (78\%)  & 6802 (541) & 2864 \\
3 & bitcoin/bitcoin & 26335 & 149.11 MB & 11 & C++ (69\%)  &4026  (452) & 946 \\
4 & dolphin-emu/dolphin & 1543 & 387.61 MB & 8 & C++ (53\%)  &1644  (144) & 539 \\
5 & django/django & 22514 & 195 MB & 9 & Python (97\%)  &3008 (215) & 415 \\
6 & xbmc/xbmc & 5533 & 1497 MB & 10 & C++ (87\%)  & 2422 (119) & 353 \\
7 & dotnet/coreclr & 2873 & 324.27 MB & 6 & C\# (80\%)  &4969  (145) & 269 \\
8 & dotnet/efcore & 2387 & 106.29 MB & 7 & C\# (99\%)  &3718  (103) & 251 \\
9 & scrapy/scrapy & 8794 & 20.17 MB & 11 & Python (100\%)  &737 (99) & 248 \\
10 & chef/chef & 2440 & 120.81 MB & 12 & Ruby (98\%)  &2080 (60) & 150 \\
11 & openzfs/zfs & 1198 & 64.33 MB & 12 & C (76\%)  &1677  (38) & 110 \\
12 & apache/camel & 4110 & 387.77 MB & 12 & Java (99\%)  &1881 (31) & 90 \\
13 & osquery/osquery & 2049 & 21.94 MB & 7 & C++ (63\%)  &895 (43)  & 79 \\
14 & apache/hadoop & 6732 & 492.81 MB & 7 & Java (93\%)  &1959  (23) & 61 \\
15 & MonoGame/MonoGame & 2404 & 82.5 MB & 10 & C\# (98\%)  &444  (7) & 33 \\
16 & composer/composer & 5905 & 16.75 MB & 10 & PHP (100\%) &515 (20) & 31 \\
17 & puppetlabs/puppet & 2158 & 78.95 MB & 11 & Ruby (99\%)  &1231  (19) & 30 \\
18 & google/jsonnet & 310 & 40.46 MB & 7 & Jsonnet (56\%)  &137  (2) & 26 \\
19 & php-webdriver/php-webdriver & 757 & 2.62 MB & 10 & PHP (97\%)  &111  (12) & 25 \\
20 & bazelbuild/bazel & 2677 & 745.4 MB & 7 & Java (84\%)  &2331  (14) & 21 \\
21 & libgit2/libgit2 & 1974 & 52.99 MB & 11 & C (98\%)  &528  (8) & 19 \\
22 & pfsense/pfsense & 1075 & 337.29 MB & 10 & PHP (94\%)  &473  (4) & 19 \\
23 & mapbox/rasterio & 365 & 24.3 MB & 8 & Python (97\%)  & 176 (11) & 18 \\
24 & aws/aws-cli & 2365 & 49.78 MB & 9 & Python (100\%)  &902  (5) & 17 \\
25 & openemr/openemr & 1078 & 453.59 MB & 11 & PHP (87\%)  &1378  (7) & 15 \\
26 & celery/celery & 3815 & 30.21 MB & 12 & Python (98\%)  &569  (9) & 12 \\
27 & fish-shell/fish-shell & 1339 & 60.2 MB & 9 & Shell (56\%)  &745  (6) & 9 \\
28 & phalcon/zephir & 448 & 20.58 MB & 8 & PHP (87\%)  &257  (4) & 9 \\
29 & h2o/h2o & 714 & 101.26 MB & 7 & C (67\%) &365  (6) & 8 \\
30 & mozilla/mozregression & 89 & 3.25 MB & 11 & Python (99\%) &253  (4) & 7 \\
31 & facebook/rocksdb & 3999 & 152.55 MB & 9 & C++ (81\%)  &2413  (7) & 7 \\
32 & phalcon/incubator & 358 & 2.39 MB & 9 & PHP (98\%) &45  (5) & 6 \\
33 & protocolbuffers/protobuf & 11808 & 61.99 MB & 7 & C++ (30\%)  &1233  (5)  & 6 \\
34 & mozilla-mobile/firefox-ios & 2265 & 514.57 MB & 7 & Swift (91\%)  &1419  (4) & 6 \\
35 & facebook/folly & 3692 & 29.57 MB & 9 & C++ (95\%)  &272  (4) & 5 \\
36 & apache/tez & 284 & 27.3 MB & 8 & Java (91\%)  &44  (1) & 5 \\
37 & libgit2/pygit2 & 317 & 6.45 MB & 11 & C (55\%) &75  (2) & 3 \\
38 & apache/hive & 3205 & 509.14 MB & 12 & Java (84\%)  &1112  (2) & 3 \\
39 & apache/maven & 1747 & 45.19 MB & 12 & Java (100\%)  &174  (2) & 2 \\
40 & mozilla/kitsune & 614 & 130.79 MB & 11 & Python (63\%)  &762  (2) & 2 \\
41 & thoughtbot/gitsh & 104 & 6.18 MB & 8 & Ruby (84\%)  &32  (2) & 2 \\
42 & aws/aws-sdk-php & 966 & 90.59 MB & 9 & PHP (99\%) &223  (1) & 2 \\
43 & mongodb/mongo & 4582 & 554.73 MB & 12 & C++ (74\%)  &101  (1) & 1 \\
44 & aws/aws-sdk-java & 2552 & 1823.94 MB & 11 & Java (100\%)  &95  (1) & 1 \\
45 & SFTtech/openage & 953 & 10.08 MB & 8 & Python (61\%)  &159  (1) & 1 \\
46 & mysql/mysql-server & 2187 & 3087.78 MB & 7 & C++ (59\%)  &80  (1) & 1 \\
% 47 & nhibernate/fluent-nhibernate & 701 & 48.33 MB & 12 & C\# (100\%) &20  (1) & 1 \\
        \bottomrule
    \end{tabular}
    \label{tab:all_repos}
\end{table*}

==> tables/variables.tex <==
\begin{table}
\caption{Dependent and independent variables.} 
\label{table:variables}
\centering \def\arraystretch{1.1}
\begin{tabular}{@{\hskip1pt}c@{\hskip2pt}| l l}
\toprule
\textbf{Type}& \textbf{Variable} & \textbf{Values}  \\
\midrule
\multirow{6}{*}{\rot{\textbf{Independent}}}  &\multirow{3}{*}{\makecell[l]{$x_1$: Usage of suggestions}}
    & No\                       
&    & Yes\\
&$x_2$: Additions & Integer\\
&$x_3$: Deletions & Integer\\
&$x_4$: Changed Files & Integer\\
&$x_5$: Commits & Integer\\
&$x_6$: PR Author Role & \makecell[l]{\\Member, \\Contributor, \\ Collaborator, \\None}\\
\midrule
\multirow{2}{*}{\rot{\textbf{Dependent}}}
& $Y_{\scaleto{MERGE}{3pt}}$: Number of Merges & Integer\\
& $Y_{\scaleto{DURATION}{2,5pt}}$: Project Duration & Integer\\
\bottomrule
\end{tabular}
% \vspace{-0.6cm}
\end{table}



